Is Solving Graph Neural Tangent Kernel Equivalent to Training Graph Neural Network?

A rising trend in theoretical deep learning is to understand why deep learning works through Neural Tangent Kernel (NTK) [jgh18], a kernel method that is equivalent to using gradient descent to train a multi-layer infinitely-wide neural network. NTK is a major step forward in the theoretical deep learning because it allows researchers to use traditional mathematical tools to analyze properties of deep neural networks and to explain various neural network techniques from a theoretical view. A natural extension of NTK on graph learning is \textit{Graph Neural Tangent Kernel (GNTK)}, and researchers have already provide GNTK formulation for graph-level regression and show empirically that this kernel method can achieve similar accuracy as GNNs on various bioinformatics datasets [dhs+19]. The remaining question now is whether solving GNTK regression is equivalent to training an infinite-wide multi-layer GNN using gradient descent. In this paper, we provide three new theoretical results. First, we formally prove this equivalence for graph-level regression. Second, we present the first GNTK formulation for node-level regression. Finally, we prove the equivalence for node-level regression.

==> uselesscode.tex <==
\begin{lemma}[Hypothesis 3]\label{lem:hypothesis_3}
Fix $\epsilon_H'>0$ independent of $t$. If for all $\tau < t$
\begin{align*}
    \| \H(0) - \H^{\cts} \| \leq 4 N n ( \log{(Nn/\delta)} / m )^{1/2} \leq \Lambda_0/4
\end{align*}
and
\begin{align*}
    \| \H(0) - \H(\tau) \| \leq \epsilon_H' \leq \Lambda_0/4
\end{align*}
and
\begin{align}\label{eq:335_2}
	4 N n ( \log ( N n / \delta ) / m )^{1/2} \leq \frac{\epsilon_{\train}}{8\kappa^2\|Y-u^*\|_2}(\kappa^2\Lambda_0 )
\end{align}
and 
\begin{align}\label{eq:335_3}
    \epsilon_H' \leq \frac{\epsilon_{\train}}{8\kappa^2\|Y-u^*\|_2}(\kappa^2\Lambda_0 )
\end{align}

then we have
\begin{align*}
    \| u_{\gnn}(t) - u^* \|_2^2 \leq \max\{\exp(-(\kappa^2\Lambda_0 )t/2 ) \cdot \| u_{\gnn}(0) - u^* \|_2^2, ~ \epsilon_{\train}^2\}.
\end{align*}
\end{lemma}

\begin{proof}
By triangle inequality we have
\begin{align}\label{eq:335_1}
    \| \H(\tau) - \H^{\cts} \| 
    \leq & ~ \| \H(0) - \H(\tau) \| + \| \H(0) - \H^{\cts} \| \notag \\
    \leq & ~ \epsilon_H' + 4 N n ( \log{(Nn/\delta)} / m)^{1/2} \notag\\
    \leq & ~ \Lambda_0/2
\end{align}
holds for all $\tau < t$. Denote $ \epsilon_H = \epsilon_H' + 4 N n( \log{(Nn/\delta)} / m )^{1/2}$, we have $\| \H(\tau) - \H^{\cts} \| \leq \epsilon_H \leq \Lambda_0/2$, which satisfies the condition of Lemma~\ref{lem:linear_converge_nn}. Thus, for any $\tau < t$, we have
\begin{align}\label{eq:induction_linear_convergence}
    \frac{ \d \| u_{\gnn}(\tau) - u^* \|_2^2 }{ \d \tau } 
    \leq & ~ - ( \kappa^2 \Lambda_0 ) \cdot \| u_{\gnn} (\tau) - u^* \|_2^2 + 2 \kappa^2 \| H(\tau) - H^{\cts} \| \cdot \| u_{\gnn} (\tau) - u^* \|_2 \cdot \| Y - u^* \|_2 \notag\\
    \leq & ~ - ( \kappa^2 \Lambda_0 ) \cdot \| u_{\gnn} (\tau) - u^* \|_2^2 + 2 \kappa^2 \epsilon_H \cdot \| u_{\gnn} (\tau) - u^* \|_2 \cdot \|Y-u^*\|_2 
    % \\
    % \leq & ~ - ( \Lambda_0 + \lambda ) \cdot \| u_{\gnn} (t) - u^* \|_2^2 ,
\end{align}
where the first step follows from Lemma~\ref{lem:linear_converge_nn}, the second step follows from Eq.~\eqref{eq:335_1}. Now let us discuss two cases:

{\bf Case 1.} If for all $\tau < t$, $\|u_{\gnn}(\tau) - u^*\|_2 \geq \epsilon_{\train}$ always holds, we want to argue that 
	\begin{align*}
		\| u_{\gnn}(t) - u^* \|_2^2 \leq \exp(-(\kappa^2 \Lambda_0 ) t/2) \cdot \| u_{\gnn}(0) - u^* \|_2.
	\end{align*}
	Note by assumption~\eqref{eq:335_2} and~\eqref{eq:335_3}, we have 
	\begin{align*}
		\epsilon_H \leq \frac{\epsilon_{\train}}{4 \kappa^2 \|Y-u^*\|_2}(\kappa^2 \Lambda_0 )
	\end{align*}
	implies
	\begin{align*}
	2 \kappa^2 \epsilon_H \cdot \|Y-u^*\|_2 \leq (\kappa^2 \Lambda_0)/2\cdot \|u_{\gnn}(\tau)-u^*\|_2
	\end{align*}
	holds for any $\tau < t$. Thus, plugging into~\eqref{eq:induction_linear_convergence},
	\begin{align*}
	    \frac{ \d \| u_{\gnn}(\tau) - u^* \|_2^2 }{ \d \tau } 
	    \leq  ~ - ( \kappa^2 \Lambda_0  )/2 \cdot \| u_{\gnn} (\tau) - u^* \|_2^2,
	    % \\
	    % \leq & ~ - ( \Lambda_0 + \lambda ) \cdot \| u_{\gnn} (t) - u^* \|_2^2 ,
	\end{align*}
	holds for all $\tau < t$, which implies
	\begin{align*}
		\| u_{\gnn}(t) - u^* \|_2^2 \leq \exp{(-(\kappa^2 \Lambda_0 )t/2)} \cdot \| u_{\gnn}(0) - u^* \|_2^2.
	\end{align*}

{\bf Case 2.} If there exist $\bar{\tau} < t$, such that $\|u_{\gnn}(\bar{\tau}) - u^*\|_2 < \epsilon_{\train}$, we want to argue that $\|u_{\gnn}(t) - u^*\|_2 < \epsilon_{\train}$.
	Note by assumption~\eqref{eq:335_2} and~\eqref{eq:335_3}, we have 
	\begin{align*}
		\epsilon_H \leq \frac{\epsilon_{\train}}{4\kappa^2\|Y-u^*\|_2}(\kappa^2\Lambda_0)
	\end{align*}
	implies
	\begin{align*}
	2\kappa^2 \epsilon_H \cdot \|u_{\gnn}(\bar{\tau}) - u^*\|_2 \cdot \|Y-u^*\|_2 \leq (\kappa^2 \Lambda_0) \cdot \epsilon_{\train}^2.
	\end{align*}
	Thus, plugging into~\eqref{eq:induction_linear_convergence},
	\begin{align*}
	    \frac{ \d (\| u_{\gnn}(\tau) - u^* \|_2^2 -\epsilon_{\train}^2)}{ \d \tau } 
	    \leq  ~ - ( \kappa^2 \Lambda_0  ) \cdot (\| u_{\gnn} (\tau) - u^* \|_2^2 - \epsilon_{\train}^2)
	    % \\
	    % \leq & ~ - ( \Lambda_0 + \lambda ) \cdot \| u_{\gnn} (t) - u^* \|_2^2 ,
	\end{align*}
	holds for $\tau = \bar{\tau}$, which implies $ e^{( \kappa^2\Lambda_0  )\tau} (\| u_{\gnn}(\tau) - u^* \|_2^2 -\epsilon_{\train}^2) $ is non-increasing at $\tau = \bar{\tau}$. Since $\| u_{\gnn}(\bar{\tau}) - u^* \|_2^2 - \epsilon_{\train}^2 < 0$, by induction, $ e^{( \kappa^2\Lambda_0   )\tau} (\| u_{\gnn}(\tau) - u^* \|_2^2 -\epsilon_{\train}^2) $ being non-increasing and $\| u_{\gnn}(\tau) - u^* \|_2^2 - \epsilon_{\train}^2 < 0$ holds for all $\bar{\tau} \leq \tau \leq t$, which implies
	\begin{align*}
	\|u_{\gnn}(t) - u^*\|_2 < \epsilon_{\train}.
	\end{align*}

Combine above two cases, we conclude
\begin{align*}
\| u_{\gnn}(t) - u^* \|_2^2 \leq \max\{\exp(-(\kappa^2\Lambda_0 )t/2 ) \cdot \| u_{\gnn}(0) - u^* \|_2^2, ~ \epsilon_{\train}^2\}.
\end{align*}
\end{proof}








%In our case, we only consider $M=1$ first since there is no inherent different between the case $M=1$ and $M>1$. We give a proof sketch of extension to multiple layers in the appendix.

%Note that the vectors $h^{(l,0)}_u \in \R^m$ for all $l \in [2:P]$, and the only special case is $h^{(1,0)}_u \in \R^d$. 
%$c_u \in \R$ is a scaling parameter, which controls weight of different nodes during neighborhood aggregation. 
% One choice of $c_u$ is to between values $ \{1, \frac{1}{|\mathcal{N}(u)|+1} \}$ \cite{dhs+19}.

% We consider two different kinds of {\readout} operation.\\

%2) Using the {\readout} operation with jumping knowledge as in \cite{xltskj18}, the final output of the GNN on graph $G$ is
%\begin{align*}
    %f_{\gnn}(G) := \sum_{u \in U} [h^{(0, Q)}_u, h^{(1, Q)}_u, \cdots, h^{(P, Q)}_u] \in \R^{m \times (P+1)}.
%\end{align*}
% When the context is clear, we also write $f_{\gnn}(G)$ as $f_{\gnn}(W, G)$, where $W$ denotes all the parameters: $W = (W^{(1,1)}, \cdots, W^{(P,Q)})$.


% Without loss of generality, we consider the GNN with exactly one $\textsc{Aggregate}$, one $\textsc{Combine}$, and one $\textsc{ReadOut}$ operation.

% we use $h(G)_v \in \R^{d}$ to denote the feature vector associated with the node $v$ in graph $G$ and $\mathcal{N}(G, u)$ to denote the neighborhood of node $u$ in graph $G$. 



Assuming there are always $N$ nodes in a graph, we use $x_i,~i\in[N]$ to denote $h_{G,u}$ associated with the $i$th node $u$ in the graph $G$ for simplify. 
Then we used a $\textsc{Combine}$ operation to learn node embedding. $\textsc{Combine}$ operation can be view as a Multi-layer perceptron, and its weight vector can be represent as $w_r \in \R^d,~r\in[m]$ or $W = [w_1, \cdots, w_m]\in\R^{d \times m}$. 
For the $\textsc{ReadOut}$ operation, node embedding are summed over all node features to get the representation $f_{\gnn}$ of an entire graph $G$. Finally, we summed over the output feature by weights $a_r \in \{-1, +1\},~r\in[m]$ or $a = [a_1, \cdots, a_m]^\top$. The weights determine whether or not change some sign of the values of the output feature when read out the representation.
% is the output weight,

% The parameters $W\in \R^{m \times d}$%^{(l,r)} 
%for all $(l,r) \in [P] \times [Q] \backslash \{(1,1)\}$, and the only special case is $W^{(1,1)} \in \R^{m \times d}$.%  $c_{\phi} \in \R$ is a scaling parameter, which is set to be $2$, following the initialization scheme used in \cite{dhs+19, hzr15}.

% After the first layer, we have the final {\readout} operation before output.

 % h^{(l,r)}_u := ( c_{\phi} /m )^{1/2} \cdot \phi(W^{(l, r)} \cdot h^{(l, r-1)}_u) \in \R^m.
 
 

% For the rest of the paper, we only consider a single-hidden-layer GNN and set  for simplicity.

% In the end of appendix section~\ref{sec:equiv_proof_sketch}\Danyang{need a forward pointer}, we show a proof sketch of how to extend our equivalence result to multi-layer GNNs.

% Let $G$ be a graph and $h(G)_v \in \R^{d}$ denote the feature vector of a node $v$ in graph $G$ where $d$ is the dimension of the feature vector. The $\textsc{Aggregate}$ operation sum up the features from neighborhood $\mathcal{N}(G, u)$ 
% associated with the node $v$ in graph $G$.

% We define the output of $\textsc{Aggregate}$ operation as follow
% \begin{align*}
% h_{G,u} := \sum_{ v \in \mathcal{N}(G,u) \cup \{u\} } h(G)_v
% \end{align*}


